SCENT: Robust Spatiotemporal Learning for Continuous Scientific Data via Scalable Conditioned Neural Fields

Spatiotemporal learning is challenging due to the intricate interplay between spatial and temporal dependencies, the high dimensionality of the data, and scalability constraints. These challenges are further amplified in scientific domains, where data is often irregularly distributed (e.g., missing values from sensor failures) and high-volume (e.g., high-fidelity simulations), posing additional computational and modeling difficulties. In this paper, we present SCENT, a novel framework for scalable and continuity-informed spatiotemporal representation learning. SCENT unifies interpolation, reconstruction, and forecasting within a single architecture. Built on a transformer-based encoder-processor-decoder backbone, SCENT introduces learnable queries to enhance generalization and a query-wise cross-attention mechanism to effectively capture multi-scale dependencies. To ensure scalability in both data size and model complexity, we incorporate a sparse attention mechanism, enabling flexible output representations and efficient evaluation at arbitrary resolutions. We validate SCENT through extensive simulations and real-world experiments, demonstrating state-of-the-art performance across multiple challenging tasks while achieving superior scalability.

==> tables/table_reconstruction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\caption{Forecasting performance comparisons on simulated and real datasets. Rel-MSE and RMSE are used for simulated and real data, respectively.}
\label{table:reconstruction}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}

\begin{tabular}{@{}llllll@{}}
\toprule
             & S1          & S2        & S3       & S4      & S5      \\ \midrule
CORAL -recon & 6.83E-02          & 1.44E-01          & 1.13E-01          & 1.38E-01          & 1.54E-01          \\
AROMA recon  & 7.13E-02          & \textbf{1.79E-01} & \textbf{1.66E-01} & \textbf{1.82E-01} & \textbf{1.87E-01} \\
SCENT        & \textbf{5.31E-02} & 2.03E-01          & 2.03E-01          & 1.99E-01          & 2.40E-01          \\ \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
